Temporal Early Exits for Efficient Video Object Detection

Transferring image-based object detectors to the domain of video remains challenging under resource constraints. Previous efforts utilised optical flow to allow unchanged features to be propagated, however, the overhead is considerable when working with very slowly changing scenes from applications such as surveillance. In this paper, we propose temporal early exits to reduce the computational complexity of per-frame video object detection. Multiple temporal early exit modules with low computational overhead are inserted at early layers of the backbone network to identify the semantic differences between consecutive frames. Full computation is only required if the frame is identified as having a semantic change to previous frames; otherwise, detection results from previous frames are reused. Experiments on CDnet show that our method significantly reduces the computational complexity and execution of per-frame video object detection up to $34 \times$ compared to existing methods with an acceptable reduction of 2.2\% in mAP.

==> Dataset.tex <==
\begin{figure}
    \centering
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={IoU},
xmin=-0.05, xmax=1.05,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Probability},
ymin=0, ymax=4.85190736055154,
ytick style={color=black}
]
\draw[draw=none,fill=color0] (axis cs:-6.93889390390723e-18,0) rectangle (axis cs:0.1,0.0256548149062409);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0};
\addlegendentry{Data}

\draw[draw=none,fill=color0] (axis cs:0.1,0) rectangle (axis cs:0.2,0.041082968200372);
\draw[draw=none,fill=color0] (axis cs:0.2,0) rectangle (axis cs:0.3,0.133740048841125);
\draw[draw=none,fill=color0] (axis cs:0.3,0) rectangle (axis cs:0.4,0.299482495658077);
\draw[draw=none,fill=color0] (axis cs:0.4,0) rectangle (axis cs:0.5,0.520678133457934);
\draw[draw=none,fill=color0] (axis cs:0.5,0) rectangle (axis cs:0.6,0.833296599635013);
\draw[draw=none,fill=color0] (axis cs:0.6,0) rectangle (axis cs:0.7,0.990134797979353);
\draw[draw=none,fill=color0] (axis cs:0.7,0) rectangle (axis cs:0.8,1.02372409172258);
\draw[draw=none,fill=color0] (axis cs:0.8,0) rectangle (axis cs:0.9,1.51134189669309);
\draw[draw=none,fill=color0] (axis cs:0.9,0) rectangle (axis cs:1,4.62086415290622);
\end{axis}

\end{tikzpicture}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}
